RLocator: Reinforcement Learning for Bug Localization

Software developers spend a significant portion of time fixing bugs in their projects. To streamline this process, bug localization approaches have been proposed to identify the source code files that are likely responsible for a particular bug. Prior work proposed several similarity-based machine-learning techniques for bug localization. Despite significant advances in these techniques, they do not directly optimize the evaluation measures. We argue that directly optimizing evaluation measures can positively contribute to the performance of bug localization approaches. Therefore, In this paper, we utilize Reinforcement Learning (RL) techniques to directly optimize the ranking metrics. We propose RLocator, a Reinforcement Learning-based bug localization approach. We formulate RLocator using a Markov Decision Process (MDP) to optimize the evaluation measures directly. We present the technique and experimentally evaluate it based on a benchmark dataset of 8,316 bug reports from six highly popular Apache projects. The results of our evaluation reveal that RLocator achieves a Mean Reciprocal Rank (MRR) of 0.62, a Mean Average Precision (MAP) of 0.59, and a Top 1 score of 0.46. We compare RLocator with two state-of-the-art bug localization tools, FLIM and BugLocator. Our evaluation reveals that RLocator outperforms both approaches by a substantial margin, with improvements of 38.3% in MAP, 36.73% in MRR, and 23.68% in the Top K metric. These findings highlight that directly optimizing evaluation measures considerably contributes to performance improvement of the bug localization problem.

==> Discussion.tex <==
\section{Discussion}

% In this section, we discuss our results further. First, we discuss about the impact of entropy regularization (Section~\ref{subsec: entropy}). Second, we discuss about the characteristics of the unrankable data (Section~\ref{subsec: unrankable}).
% \label{sec:discussion}
% %  \begin{figure}[ht!]
% %     \centering
% %     \includegraphics[scale=0.30]{Figures/Length_Distribution.eps}
% %     \caption{Source code length distribution.}
% %     \label{fig:length distro}
% % \end{figure}
% \noindent
%
% \subsection{Unrankable Data in RLocator.}
\label{sec: unrankable}
% As discussed in Section~\ref{sec:ranking}, we limit the number of states in RLcoator to 31, which led to removing 15\% of the initial dataset.
% % That is, we remove 15\% of the initial dataset of bug reports.
% In such data, ElasticSearch (ES) fails to correctly rank the file relevant to a given bug within the top 31$^{st}$ files, i.e., for 15\% of the bug reports, ES was unable to place any relevant files to the bug within the top 31$^{st}$ positions.
% Consequently, such data is not useful for the model, given no relevant files to the bug will appear in the candidate files.
% Also, including such data in the model can be misleading to developers as the model will not produce meaningful results.
% Hence, as an initial step of RLocator, it is important to filter out data that ES would fail to rank properly (we refer to this data as unrankable data).

% Since we obtain ground truth of the bug reports in our dataset (Provided by Ye et al.~\cite{Ye2014}), it was possible to identify unrankable data in our initial dataset, i.e., we check if the candidate files (the 31 files) suggested by ES include any relevant files by cross-referencing with the obtained ground truth.
% % If the set of files includes at least one relevant file to the bug, the set is passed to the RL model for training.
% % Otherwise, the set is excluded from the model training data.
% However, in the real-world scenario (assuming that we put RLocator in production environment), it is not possible to verify whether the candidate files suggested by ES include any relevant file (as no ground truth would be available in this scenario).
% Hence, to put our model into action, we need to identify the candidate set of unrankable data that should be filtered out.
% % Hence, to put things in a more realistic action, our goal in this section is to provide a method that help identify such potentially unrankable data.
% % we sampled 20 bugs from each project's unrankable data and 

% %Approach
% \input{Tables/Features.tex}
% To determine our set of candidates, we study the most important features associated with unrankable data.
% We consult the related literature on the field of information retrieval~\cite{Lv2011, Lv2011_plus, Lewis1998} and bug report classification~\cite{Fang2021} for feature selection.
% We describe the list of computed features in Table~\ref{table:feature_description}.
% % ThTables/Features.texefore, we sampled 20 bugs from each project's unrankable data and manually checked them to identify come characteristics of those data (bug reports).
% % In Section~\ref{sec:ranking} we have said that we can not use 15\% of the data. Still, we need to identify the 15\% data to filter out.
% We compute the selected features for our dataset of bug reports.
% Then, we build an XGBoost-based binary classifier model~\cite{Chen2016} to identify  data points that a textual similarity-based ranking system (e.g., ES) can not rank correctly. 
% We train the classifier to predict whether the bug is rankable or not.

% The classifier model achieves a precision of 0.82, a recall of 0.93, and an F1-score of 0.85.
% The confusion matrix for the model has been presented in Table~\ref{table:confusion_matrix}
% \input{Tables/Confusion_Matrix.tex}

For using RLocator effectively in real-world scenarios, we have used an XGBoost model (Section~\ref{sec: identification_of_unrankable_data}). The XGBoost model filters out the bug reports where the relevant files do not appear in the top $k$ (=31) files. Moreover, to understand the characteristics of the bug reports and the associated 31 retrieved files, we computed the importance of our selected features mentioned in Table~\ref{table:feature_description}.
XGBoost offers a built-in module to calculate the importance.
The importance score indicates how much each feature contributes to the model.
% or valuable
% each feature was in the construction of the model. 
We report the default type of importance,  ``weight''. 
A higher value of this metric implies that the feature is more important for generating a prediction. 
Figure~\ref{fig:feature_importance} shows the importance of our selected features. The figure shows that the most important feature is Similarity, followed by Source Code Length, Bug Report Length, and Stack Trace. Our findings are aligned with previous studies~\cite{Rahman2018} that state: \emph{similarity of a bug report is a major factor to consider when using text-based search systems.}
\par
To understand the characteristics of the bugs for which no relevant files appear in the top $k$ files, we manually checked them. We have sampled ten bug reports for each project and looked for a common pattern. We find three noticeable patterns in those bug reports. The first one is vague bug report. For example, 
\bugreportquote{``Allow to disable icons in vertical ruler I2003 does not appear''}{JDT-45509}
The report describes certain UI feature that does not appear. However, the context is missing from the bug report. A developer who is accustomed to the product may be able to localize the bugs, but for a textual similarity-based system, this bug is very hard to localize without the necessary context.


\begin{figure}[tb!]
    \centering
    \includegraphics[scale=0.16]{Figures/Feature_Importance.pdf}
    \caption{Feature importance of classifier model.}
    \label{fig:feature_importance}
\end{figure}
% \begin{figure}[tb!]
%     \centering
%     \includegraphics[scale=0.16]{Figures/Feature_Importance.eps}
%     \caption{Feature importance of classifier model.}
%     \label{fig:feature_importance}
% \end{figure}
The second pattern is the length of a bug report is too short to have any information to localize bugs. For example, in `JDT-26261', we have only the title of the bug report and no description or details of the bug. The title of the bug report is,
\bugreportquote{``Confusion after setting hover prefs due to disabled hover - remove hover toggle''}{JDT-26261}

The third one is media attachment. In the description field, some media is attached, where the actual problem has been explained. For example, in 
\bugreportquote{``One of our customized reports has a cross tab with filter applied. Before upgrade(BIRT Report Designer v2.3.2), the cross tab can display filtered data without any problem. After upgrade(BIRT Report Designer v3.7.1), the cross tab data can no longer be displayed in the screenshot below:
[testing rptdesign script attached]''}{Birt-419097}
Text-based search systems are not designed to utilize any kind of media (e.g., image, video). Thus, it is tough for them to rank any relevant files in the top $k$ results. Further research on bug localization tools could explore the potential use of attachments in bug localization.

Zimmermann et al.~\cite{Zimmermann2010} have identified three key characteristics of an effective bug report, including the inclusion of code samples/stack traces, readability, and a clear description of attachments. Thus if bug reports have these characteristics, then developers may be able to effectively use automated bug localization tools such as ours.

%Maybe developers should also keep in mind the characteristics while using automated bug localization. 
% \mei{Are you going to update the next sentence?}
% Such observation points out that \emph{similarity of a bug report is a major factor to consider when using text-based search systems.}
%
% Table XX presents the findings of the features importance derived from the classifier model. 
% All the features are ordered on the basis of their explanatory power(x2). 
% With each independent feature, we report its estimated
% coefficient, its explanatory power (x2), its p-value, and its statistical significance code (using asterisks).
% Our results reveal that the most important feature is Source code length, followed by similarity, bug report length, and stack trace. 
% Such observation points out that \emph{source code length is a major problem using text-based search systems.}\par

% We have also calculated feature importance for all the features, and the most important feature is Source code length, followed by similarity, bug report length, and stack trace. The observation points out that \emph{source code length is a major problem using text-based search systems.}\par

% In the first step of building the model, we sampled 20 bugs from each project's unrankable data and manually checked them to identify features.
% From manual checking, we found three features that might contribute to the cause.
% Also, we have included one feature that has been found impactful in previous studies~\cite{Schroter2010}. 

% The features are described below,
% \begin{itemize}
%     \item \textbf{Bug Report Length:} Here, we have calculated the length of bug reports. If the bug report does not contain enough information, it would be tough to find textual similarity. This feature will give us a sense of the amount of information in the bug report.
%     \item \textbf{Source Code Length (Median):} Each bug report is associated with a specific state/version of the code repository. We have calculated the length of all the source codes in that particular version and picked the median length as one of the features. Often it is tough for textual similarity rankers to estimate similarity for long text~\cite{Lv2011}. That is why we included this feature.
%     \item \textbf{Stack-trace:} Schroter et al.~\cite{Schroter2010} have found that bug reports can help the debugging process by containing useful information, which is why we included this feature. This is a binary feature. We have checked whether the bug report includes any stack trace or not. 
%     \item \textbf{Similarity:} In our manual checking, we noticed that if the bug report explains the problem using technical domain terms, the text search method is more likely to rank the buggy file. To use the ``technical domain word usage" property as a feature, we used the \emph{similarity} feature. To calculate the similarity, first, we have tokenized the bug report and all the source code (of that particular version). Then following equation~\ref{eq:similarity}, we calculated the similarity. After that, we picked up the median similarity score as a feature.
%     \begin{equation}
%     \label{eq:similarity}
%     \hspace*{-2em}
%         Similarity = \frac{Bug\ Reports\ Token \cap Source\ Codes\ Token}{\#\ of\ Unique\ Tokens\ in\ Bug\ Report}
%     \end{equation}
% \end{itemize}

% \textbf{Validation of source code length feature.}
% \begin{figure}[tb!]
%     \centering
%     \includegraphics[scale=0.16]{Figures/BM25_Performance.eps}
%     \caption{Performance of the BM25 variants.}
%     \label{fig:BM25 variants}
% \end{figure}
% So far, we empirically find that Similarity is the most influential feature that can distinguish whether a source code file will appear in the top $k$ by a text-based search system or not.
% However, it is still unclear how the similarity would impact retrieved documents' ranking in practice, i.e., we want to identify the threshold of similarity, after which the performance of text-based search systems (i.e., ES) would drop.

% To that end, we experiment with several popular similarity measurement techniques (e.g., TF-IDF or BM25) that ES employs for calculating the similarity between queries and documents.
% % to identify the source code lengths limit, after which the text-based similarity search methods' performance drop.
% % Text-based search systems usually use TF-IDF or BM25 for calculating the similarity between queries and documents.
% Previous studies proposed different variants of BM25.
% For example, BMOkapi~\cite{Schroter2010} is the naive version of BM25. 
% Other more advanced techniques include BM25L~\cite{Lv2011} and BM25+~\cite{Lv2011_plus}.
% % to address the problem. 
% We use the three techniques to measure the retrieval performance across different source code file lengths in our dataset. 
% We use the implementation proposed by prior work (i.e., ~\cite{Lv2011, Lv2011_plus,Robertson1994}
% for using the BM25 variants.
% % Yuanhua et al.~\cite{Lv2011, Lv2011_plus} and Robertson et al.~\cite{Robertson1994}
% % , we have used the parameters proposed by Yuanhua et al.~\cite{Lv2011, Lv2011_plus} and Robertson et al.~\cite{Robertson1994}. 
% % For implementing the BM25 variants, we have used the parameters proposed by Yuanhua et al.~\cite{Lv2011, Lv2011_plus} and Robertson et al.~\cite{Robertson1994}. 

% To collect a dataset of varying source code lengths, we first identify the distribution of the source code length of files associated with bug reports in our dataset. 
% Then, we create a randomly selected sample of 2,500 bug reports from each quartile of the data. 
% Note that the number of bug reports is not equally distributed across the four quantiles, e.g., the total number of bugs in the 3rd Q is 3,236.
% % We obtain a number of 25 bugs from each Q.
% Since bug reports are associated with source codes of different lengths, it is challenging to select bug reports with the same median source code lengths.
% % getting a bug report with a specific source code length is challenging.
% Thus, we consider $\pm 10$\% variance of the length. 
% For example,  the second quartile of source code length is 4,233. 
% Hence, we sample 2,500 bug reports with source code lengths ranging between 3,810 and 4,656.
% Finally, we evaluate the performance of different BM25 variants. 

% Figure~\ref{fig:BM25 variants} presents the performance of the BM25 variants.
% We can see from Figure~\ref{fig:BM25 variants} that BM25L achieves the highest performance, followed by BM25Plus and BM25Okapi (default BM25). 
% However, the performance of BM25L starts to drop when the source code length is more than 8,300. Our analysis points out that a bug localization tool is more likely to fail if the similarity of the bug report. Thus, \emph{developers should identify the cases based on source code length and handles them manually.}
% The BM25L has been designed to accommodate long documents (source code files). Still, we found that its performance drops after a certain threshold. The observation points out \emph{the need for a new technique to handle long files.} 
%developer should handle more than 8300
% 1. still fail bm25l
%2.  more advnaced approaches
% Such result points out that \emph{as source code length increases, the retrieval performance of BM25 decreases}

==> Prev_Background.tex <==
\section{Background}
\label{sec:background}
In this study, we used two reinforcement learning algorithms,  DQN and A2C (with entropy), with entropy to develop the RL agent. These two algorithms are representative of two major categories of reinforcement learning algorithms: policy optimization and value optimization-based algorithms. We have chosen DQN and A2C (with entropy) as they are less complex, comparatively highly efficient in convergence, and more interpretable. A brief description of terms used in this study and the two algorithms is presented below.

In Reinforcement learning, the agent has been trained to identify the best action in a giver state. The agent's strategy to determine the best action which will eventually lead to the highest cumulative reward is referred to as \emph{policy}.\par
\emph{Q value} refers to the cumulative reward (until the goal/end) that an agent can get if it takes a specific action in a certain state. The function that is used to estimate the \emph{Q value} is often referred as \emph{Q function} or \emph{Value function}.\par
In RL, an agent starts its journey from a starting state, and then it continues to go forward by picking appropriate action. The journey will end in a pre-defined end state. The journey from start to an end state is referred to as \emph{episode}.

\subsection{Value Optimization}
The agent tries to learn the Q value function in value optimization approaches. The approach can also be categorized as off-policy algorithm. The agent will keep the Q value function in memory and update it gradually. It will consult the Q value function in a particular state and pick the action that will give the highest value (reward).

\subsection{Policy Optimization}
In the Policy optimization approach, the agent tries to learn the mapping between state and the action that will result in the highest reward. The agent will pick the action based on the mapping in a particular state.

\subsection{Deep Q Network (DQN)} Depp Q Network utilizes a neural architecture to estimate the value of the q function. The target of the DQN has been calculated by using  equation~\ref{eq:qnet}. 

\begin{equation}
    \label{eq:qnet}
    Value_{Target} = R(S,A,S') + \gamma \; \underset{a'}{max}(Q(S',A', \theta)
\end{equation}


Here, $R(S,A,S')$ represents the reward received while changing current state from $S$ to $S'$ using action $A$ and $Q(S',A', \theta)$ represents the Q network the predicts the future reward received from current state $S'$ using action $A'$, $\theta$ represents the parameters of the Q network.  Then the DQN learns the future return of a current action by optimizing the target value. However,  DQN tries to optimize the loss using its own predicted value of the future state, which leads to an unstable weight update. Thus in Double DQN (DDQN), two different networks (Q network, target Q network) has been used for Q value estimation. In double DQN the equation~\ref{eq:dqnet} become
\begin{equation}
    \label{eq:dqnet}
    Value_{Target} = R(S,A,S') + \gamma \; (Q(S', \underset{a'}{max}Q(S',A,\theta), \theta')
\end{equation}

Most of the real-world MDP problems are partially observable Markov decision processes. As the agent can not observe the states thoroughly, previous studies~\cite{Hausknecht2015} have suggested using recurrent units inside the deep Q network helps to understand the unobserved states by learning from the previous steps. In that case the MDP problem become  $\langle S, A, \tau, \Re, \pi, \Omega\rangle$ One of the requirements of the agent training in this study is that they are not allowed to take the same action twice. Thus, we used a double deep recurrent Q network in this study (DDRQN). From now on, we will refer to this network as simply DQN.


\subsection{Advantage Actor Critic (A2C) with entropy} A2C is a policy-based algorithm where the agent learns an optimized policy to solve a problem. A2C algorithm utilizes the advantage of a particular state, action pair to determine the best possible action using equation~\ref{eq:gen_ad}. Here, $V^{\pi}(S)$ represents the value model which predicts the possible value of state $S$ where $Q^{\pi}(S, A)$ estimates the potential Q value of the state-action pair. Intuitively advantage represents how much extra reward can be earned using a particular action $A$ in state $S$ compared to the average reward received in state $S$. However, in this study we have used temporal difference (TD) advantage using equation~\ref{eq:td_ad}
\begin{equation}
    A^{\pi}(S, A) = Q^{\pi}(S, A) - V^{\pi}(S) \label{eq:gen_ad}
\end{equation}
\begin{equation}
    A^{\pi}(S, A) = R(S, A, S') + \gamma V^{\pi}(S') - V^{\pi}(S) \label{eq:td_ad}
\end{equation}

In Actor-Critic, the Actor-network picks action. The future return of action is estimated using the critic network. The actor-network uses the critic network to pick the best action in any state. Advantage actor-critic subtracts a base value from the return in timestep t. A2C with entropy adds the entropy of the probability of the possible action with the loss of the actor-network. As a result, in the gradient descent step, the model tries to maximize the entropy of the learned policy. Maximization of entropy makes sure that the agent assigns an almost equal probability to an action with a similar return. In this study, we trained an RL agent for the ranking task. The agent will rank buggy files from a set of files based on the bug report. However, there can be more than one buggy file for one bug report. Thus, it is desired that the buggy files be in the least indices and all buggy files be ranked closer to each other.

==> Prev_Formulation.tex <==
\section{Ranking as Markov Decision Process}
\label{sec:ranking}
The process of bug localization can be defined as a Markov Decision Process (MDP) where the ranking system is just a sequence of decision-making steps. In each timestep, the ranking system will choose a document from the list of available documents. The reinforcement learning model can be represented by a tuple $\langle S, A, \tau, \Re, \pi\rangle$ composed by states, actions, transition, reward, and policy, which are respectively defined as follows:
\begin{itemize}
    \item \textbf{States:} $S$ is the set of states. The RL model must know the list of available documents in any step. In this study, we have created the state by concatenating the bug report's embedding with the candidate file's embedding and then stacking all the concatenated vectors together. Suppose we have two candidate files. The embedding of the bug report is $\langle Y_1, Y_2, ..., Y_n \rangle$ and the embedding of the source code is $\langle X_1, X_2, ..., X_n\rangle$, $\langle Z_1, Z_2, ..., Z_n\rangle$. Then the state will be $\langle Y_1, Y_2, ..., Y_n, X_1, X_2, ..., X_n \rangle$ and  $\langle Y_1, Y_2, ..., Y_n, Z_1, Z_2, ..., Z_n\rangle$ stacked together. The bug report is in natural language with words from the programming language domain where as source code are in the programming language. Thus we need a multi-modal embedding to project them into the same embedding space. In this study, for embedding, we have used CodeBERT~\citep{feng2020}. CodeBERT is a BERT-based transformer trained on documentation and source code pairs. We can use CodeBERT to embed both bug reports and source code as it is trained on multi-modal data. In this study, all the states between the initial state and the terminal state have been referred to as \emph{episode}.
    \item \textbf{Actions:} We defined action as picking up a document from the available  document list to the ranked list. Suppose in timestep $t$; the RL model picked the document $d$ then the rank of that particular document will be $t$. That means the number of actions and the number of timesteps will be the same in any trajectory. For this study, we have limited the number of actions to 31. The details of the reason behind this choice will be discussed in the Section~\ref{sec:methodology}.
    \item \textbf{Transition:} $\tau$(S, A) is a function $\tau$ : S × A → S which maps a state $s_t$ into a new state $s_{t+1}$ in response to the selected action $a_t$ . Choosing an action $a_t$ means removing the document out of the candidate set.
    \item \textbf{Reward:} A reward is a value provided to the RL agent as feedback on their action. Often the reward received from one action is referred to as \emph{return}. For reward we have chosen the following function.
    
        \begin{multline}
            \Re(S,A) = \frac{ M * document\; relevance}{\log_2 t * distance(s)};if \;a \;related \\document \;has \;already \;been \;picked \\
        \end{multline}
        \begin{equation}
            \Re(S,A) = -\log_2 t ; otherwise
        \end{equation}
    
    \begin{multline}
        distance (S) = Avg. (Distance\; between\;\; currently\\ picked\; subsequent\; related\; documents)
    \end{multline}
    
    \begin{figure*}[ht!]
        \centering
        \includegraphics[scale=0.40]{Figures/AspectJMultiplicator.eps}
        \caption{Effect of M in reward-episode graph}
        \label{fig:effect_m}
    \end{figure*}

    Suppose, in  State $S_i$ the currently picked documents are $P_1, P_2, P_3, P_4, P_5, P_6$ and their relevancy to the bug report is $\langle 0, 0, 1, 0, 1, 1\rangle$. Then the distance between subsequent related documents are $\langle 1, 0 \rangle$ and $distance(S_i) = 0.5$. If the agent has picked a new relevant document, we have rewarded the agent $M$ times the reciprocal rank of the document divided by the distance between the already picked related documents. We have used different values (1, 3, 6, and 9) as the value of $M$ and developed an RL model for the AspectJ project to observe the effect of $M$.  The training of each model takes more than three days to complete. The resulting smoothed reward-episode graphs (moving average of 100 episodes) have been presented in Figure~\ref{fig:effect_m}. From Figure~\ref{fig:effect_m} we can observe that using 1 as the value of $M$ resulted in an unstable reward-episode graph (reward is changing too frequently)  which finally converged into some local maxima. Using 3, 6, and 9 as $M$'s value resulted in a stable graph. However, it seems that the use of 6 and 9 resulted in a late convergence. Moreover, the reward-episode graph for 6 and 9 is almost similar. Thus, we have not conducted any further experiments by increasing the value. We have accepted 3 as the value of $M$ as it resulted in a stable graph and achieved the highest reward. As per the requirement, the agent cannot pick an already picked document. We have achieved the requirement by masking, which will be discussed in Section~\ref{sec:methodology}.

\end{itemize}

==> Prev_Methodology.tex <==
\section{Methodology}
\label{sec:methodology}
 \begin{figure*}[ht]
    \centering
    \includegraphics[scale=0.45]{Figures/Methodoloy.png}
    \caption{Methodology of the study}
    \label{fig:method}
\end{figure*}
In this study, we have developed two learning to rank models using the reinforcement learning technique. The two models differ based on how they optimize the Markov decision process. The methodology of this study has been presented in Figure~\ref{fig:method}. 

\paragraph*{\textbf{Dataset Split }} For this study, we have used the dataset provided by Ye at al.~\cite{Ye2014}. The dataset contains six projects. For each project, we first sorted the data using the reporting timestamp of the bug reports. After that, we divided them into 60: 40 splits. The first 60\% of the data is for training, and the rest 40\% of the data is for testing.

\input{Tables/Coverage_Experiment}
\paragraph*{\textbf{ElasticSearch Index}} The dataset consists of bug reports and source code files at the specific version (or commit point in a version control system) when the bug report has been filed. The number of source code files for a bug report is a variable. However, in this study, the number of actions must equal the number of source code files. As we can not have a variable number of source code files, we have shortlisted the source code files and created a fixed-size set of candidate files. We have used ElasticSearch (a text-based search engine) index for this shortlisting purpose. We built an ElasticSearch index using the source code files and then queried it into the index using the bug report. Later, we picked the first $K$ files, which have textual similarities with the bug report. ElasticSearch uses the BM25 model to estimate the textual similarity. Though a BM25 model is not good enough for bug localization, it is sufficiently good to locate related documents. Besides the text of the source code files, we have also indexed the names of the methods, classes, and interfaces implemented in those files. For extracting the name of the method, class, and interface, we have used SrcML~\cite{Collard2013}. Later we used those names along with the BM25 model to rank source code files. We have run a few experiments to identify the appropriate value of $K$. The experiments' results are presented in Table~\ref{table: coverage}. Table~\ref{table: coverage} represents the value of $K$ along with cases in percentage where the buggy files are in the Top $K$ files. The GPU size also limits the number of candidate files. We have mentioned in Section~\ref{sec:ranking} that we formulated \emph{state} using the embedding of all the candidate files. That implicates that a higher number of candidate files will lead to a larger \emph{state} and the size of \emph{state} is limited by the GPU size. We have conducted this study on an Nvidia V100 16 GB GPU. Based on the coverage and the size of GPU, we have decided that 31 as the value of $K$ is suitable for our case. We have dropped the other 15\% of the data from our train dataset. That means we have used 51\% (60*0.85) of our entire dataset as the effective train dataset. 


\paragraph*{\textbf{Embedding}} For using the text input in a deep learning model, we have to convert them into a vector. Thus, after getting the related 31 files for each bug report, we projected the bug report and the source code into vector space using the CodeBERT model. The embeddings generated in this step are used in creating states which will be used to train the reinforcement learning model. 

\paragraph*{\textbf{RL agent training}} Later in the fourth step, we used the embedding to train the RL agent (model). We have used Advantage Actor Critic (A2C) algorithm to train the model.two different RL techniques in this study. However, the architecture of both models is similar. Following the previous studies~\cite{Liang2019, Huo2021, Huo2016} the \emph{states} are passed through a Convolutional Neural Network followed by an LSTM. We have used LSTM because we wanted the RL agent to be aware of the previous states. The benefit of the awareness will help the agent not to pick already picked documents. Then, we followed the training techniques of A2C (with entropy) and DQN to train the individual model. However, our experiment found that state awareness through LSTM is slow because the model learns about invalid steps (picking a document that has already been picked) by making mistakes. Learning from errors takes a long time to converge. Thus, we have used masking to meet the requirement that the agent is not allowed to take a particular action more than once. In DQN, we have implied that condition by masking the $Q$ values with the available actions. However, in A2C, it has been achieved by masking the output before calculating the softmax probability of actions. 


\paragraph*{\textbf{Evaluation}} Finally, we have evaluated the trained RL agents on the hold-out test dataset using MRR and MAP. Similarly to the train configuration, we have used 85\% of the test data, which indicates the effective test dataset is 34\% of the entire dataset.
 \begin{equation}
 \label{eq:mrr}
     MRR = \frac{1}{n}\sum_{i=1}^n \frac{1}{\text{highest ranked buggy file for $report_i$}}
 \end{equation}
 \begin{equation}
 \label{eq:map}
     MAP = \frac{1}{n}\sum_{i=1}^n AvgP(i)
 \end{equation}

==> Tables/Confusion_Matrix.tex <==
\begin{table}[!tb]
\caption{Confusion matrix.}
\begin{tabular}{cc|cc}
\multicolumn{2}{c}{}
            &   \multicolumn{2}{c}{Predicted} \\
    &       &   Yes &   No              \\ 
    \cline{2-4}
\multirow{2}{*}{\rotatebox[origin=c]{90}{Actual}}
    & Yes   & 3387   & 347                 \\
    & No    & 820    & 427                \\ 
    \cline{2-4}
\end{tabular}
\label{table:confusion_matrix}
\end{table}
% \setlength\tabcolsep{0pt}
% \begin{tabular}{c >{\bfseries}r @{\hspace{0.7em}}c @{\hspace{0.4em}}c @{\hspace{0.7em}}l}
%   \multirow{10}{*}{\parbox{1.1cm}{\bfseries\raggedleft Actual\\ Label}} & 
%     & \multicolumn{2}{c}{\bfseries Prediction Label} & \\
%   & & \bfseries P & \bfseries N & \bfseries total \\
%   & P & \MyBox{16937} & \MyBox{1737} & 18674 \\[2.4em]
%   & N & \MyBox{4100} & \MyBox{2137} & 6237 \\
%   & total & 21037 & 3874 &
% \end{tabular}

==> Tables/Coverage_Experiment.tex <==
\begin{table}[]
\caption{Value of $K$ and coverage of the related files}
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{K} & \textbf{Coverage (\%)} \\ \hline
15         & 49.2                  \\ \hline
20         & 60                    \\ \hline
25         & 73.45                 \\ \hline
30         & 81.67                 \\ \hline
31         & 85.04                 \\ \hline
33         & 87.4                  \\ \hline
35         & 88                    \\ \hline
50         & 92.19                 \\ \hline
\end{tabular}
\label{table: coverage}
\end{table}

==> Tables/Performance_Limit.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[tb!]
\centering
\caption{Performance estimation.}
\setlength\tabcolsep{5pt}
\begin{tabular}{c|rrrl|rrrl}
\toprule
\multirow{2}{*}{\textbf{Project}} & \multicolumn{4}{c|}{\textbf{MAP}}                                                                                                                                                           & \multicolumn{4}{c}{\textbf{MRR}}                                                                                                                                                                                         \\ \cmidrule{2-9} 
                                       & \multicolumn{1}{c|}{\textbf{MAP$_{Best}$}} & \multicolumn{1}{c|}{\textbf{MAP$_{2^{nd} Worst}$}} & \multicolumn{1}{c|}{\textbf{MAP$_{Worst}$}} & \textbf{MAP \textgreater MAP$_{Worst}$}                                    & \multicolumn{1}{c|}{\textbf{MRR$_{Best}$}} & \multicolumn{1}{c|}{\textbf{MRR$_{2^{nd} Worst}$}} & \multicolumn{1}{c|}{\textbf{MRR$_{Worst}$}} & \textbf{MRR \textgreater MRR$_{Worst}$}                                                                  \\ \midrule
AspectJ                                & \multicolumn{1}{r|}{0.57}            & \multicolumn{1}{r|}{0.47}           & \multicolumn{1}{r|}{0.47}              & None                                                                  & \multicolumn{1}{r|}{0.59}            & \multicolumn{1}{r|}{0.5}            & \multicolumn{1}{r|}{0.5}               & \begin{tabular}[c]{@{}l@{}}DeepLoc, CAST,\\ KGBugLocator\end{tabular}                               \\ \midrule
Birt                                   & \multicolumn{1}{r|}{0.47}            & \multicolumn{1}{r|}{0.412}          & \multicolumn{1}{r|}{0.41}              & None                                                                  & \multicolumn{1}{r|}{0.49}            & \multicolumn{1}{r|}{0.41}           & \multicolumn{1}{r|}{0.4}               & None                                                                                                \\ \midrule
\shortstack{Eclipse\\Platform\\ UI}                    & \multicolumn{1}{r|}{0.55}            & \multicolumn{1}{r|}{0.43}           & \multicolumn{1}{r|}{0.43}              & FLIM                                                                  & \multicolumn{1}{r|}{0.59}            & \multicolumn{1}{r|}{0.52}           & \multicolumn{1}{r|}{0.51}              & DeepLoc, FLIM                                                                                       \\ \midrule
JDT                                    & \multicolumn{1}{r|}{0.51}            & \multicolumn{1}{r|}{0.44}           & \multicolumn{1}{r|}{0.44}              & CAST                                                                  & \multicolumn{1}{r|}{0.53}            & \multicolumn{1}{r|}{0.47}           & \multicolumn{1}{r|}{0.47}              & DeepLoc, FLIM                                                                                       \\ \midrule
SWT                                    & \multicolumn{1}{r|}{0.48}            & \multicolumn{1}{r|}{0.44}           & \multicolumn{1}{r|}{0.44}              & FLIM                                                            & \multicolumn{1}{r|}{0.51}            & \multicolumn{1}{r|}{0.45}           & \multicolumn{1}{r|}{0.42}              & \begin{tabular}[c]{@{}l@{}}BugLocator, CAST,\\ DeepLoc, FLIM,\\ KGBugLocator,\\ FBL-BERT\end{tabular} \\ \midrule
Tomcat                                 & \multicolumn{1}{r|}{0.59}            & \multicolumn{1}{r|}{0.52}           & \multicolumn{1}{r|}{0.52}              & \begin{tabular}[c]{@{}l@{}}DeepLoc, CAST,\\ KGBugLocator\end{tabular} & \multicolumn{1}{r|}{0.62}            & \multicolumn{1}{r|}{0.5}            & \multicolumn{1}{r|}{0.5}               & \begin{tabular}[c]{@{}l@{}}DeepLoc, CAST,\\ KGBugLocator,\\ FLIM\end{tabular}                         \\ \bottomrule
\end{tabular}
\label{table: performance estimation}
\end{table*}

==> Tables/Performance_Limit_Old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[tb!]
\centering
\caption{Performance estimation.}
\begin{tabular}{l|r|r}
\toprule
\textbf{Project Name} & \textbf{MAP Limits}                 & \textbf{MRR Limits}                \\ \midrule
AspectJ               & \textless{}0.47,0.47\textgreater{}  & \textless{}0.5,0.5\textgreater{}   \\ 
Birt                  & \textless{}0.41,0.412\textgreater{} & \textless{}0.4,0.41\textgreater{}  \\ 
Eclipse Platform UI   & \textless{}0.43,0.43\textgreater{}  & \textless{}0.51,0.52\textgreater{} \\ 
JDT                   & \textless{}0.44,0.44\textgreater{}  & \textless{}0.47,0.47\textgreater{} \\ 
SWT                   & \textless{}0.44,0.44\textgreater{}  & \textless{}0.42,0.45\textgreater{} \\ 
Tomcat                & \textless{}0.52,0.52\textgreater{}  & \textless{}0.5,0.5\textgreater{}   \\ \bottomrule
\end{tabular}
\label{table: performance estimation}
\end{table}

==> Tables/result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[tb!]
\centering
\caption{RLocator performance.}
\begin{tabular}{l|l|r|r}

\toprule
\textbf{Project Name}                & \textbf{Model} & \textbf{MAP}  & \textbf{MRR}  \\ 
\midrule
\multirow{8}{*}{AspectJ}             & RLocator       & \textbf{0.57} & \textbf{0.59} \\  
                                     & BugLocator     & 0.22          & 0.41          \\ 
                                     & DeepLoc        & 0.42          & 0.51          \\  
                                     & CAST           & 0.42          & 0.54          \\  
                                     & KGBugLocator   & 0.42          & 0.55          \\  
                                     & BL-GAN         & 0.34          & -             \\ 
                                     & FBL-BERT       & 0.08          & 0.17          \\ 
                                     & FLIM           & 0.39          & 0.47          \\ \midrule
\multirow{8}{*}{Birt}                & RLocator       & \textbf{0.47} & \textbf{0.49} \\  
                                     & BugLocator     & 0.26             & 0.30            \\ 
                                     & DeepLoc        & -             & -             \\  
                                     & CAST           & -             & -             \\  
                                     & KGBugLocator   & -             & -             \\  
                                     & BL-GAN         & -             & -             \\  
                                     & FBL-BERT       & -             & -             \\  
                                     & FLIM           & 0.23          & 0.28          \\ \midrule
\multirow{8}{*}{Eclipse Platform UI} & RLocator       & \textbf{0.55} & \textbf{0.59} \\  
                                     & BugLocator     & 0.24          & 0.32          \\  
                                     & DeepLoc        & 0.43          & 0.53          \\  
                                     & CAST           & -             & -             \\  
                                     & KGBugLocator   & -             & -             \\  
                                     & BL-GAN         & 0.32          & -             \\  
                                     & FBL-BERT       & -             & -             \\  
                                     & FLIM           & 0.5          & 0.54          \\ \midrule
\multirow{8}{*}{JDT}                 & RLocator       & \textbf{0.51} & \textbf{0.53} \\  
                                     & BugLocator     & 0.14             & 0.20             \\  
                                     & DeepLoc        & 0.44          & \textbf{0.53} \\  
                                     & CAST           & 0.47          & 0.39          \\  
                                     & KGBugLocator   & 0.4           & 0.47          \\  
                                     & BL-GAN         & 0.32          & -             \\  
                                     & FBL-BERT       & 0.06          & 0.36          \\  
                                     & FLIM           & 0.40          & 0.52          \\ \midrule
\multirow{8}{*}{SWT}                 & RLocator       & \textbf{0.48}          & 0.51          \\  
                                     & BugLocator     & 0.43          & 0.48 \\  
                                     & DeepLoc        & 0.40          & 0.49          \\  
                                     & CAST           & 0.42          & 0.50          \\  
                                     & KGBugLocator   & 0.43          & 0.51          \\  
                                     & BL-GAN         & -             & -             \\  
                                     & FBL-BERT       & 0.12          & 0.51          \\  
                                     & FLIM           & 0.45          & \textbf{0.52}          \\ \midrule
\multirow{8}{*}{Tomcat}              & RLocator       & \textbf{0.59} & \textbf{0.62}          \\  
                                     & BugLocator     & 0.24             & 0.32             \\  
                                     & DeepLoc        & 0.56          & \textbf{0.62} \\  
                                     & CAST           & 0.55          & 0.61          \\  
                                     & KGBugLocator   & 0.56          & \textbf{0.62} \\  
                                     & BL-GAN         & 0.45          & -             \\  
                                     & FBL-BERT       & 0.13          & 0.43          \\  
                                     & FLIM           & 0.53          & 0.61          \\ 
\bottomrule
\end{tabular}

\label{table:result}
\end{table}

==> Tables/result3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[tb!]
\centering
\caption{RLocator performance.}
\begin{tabular}{l|l|ccc|ccc}
\hline
\multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Project Name}}} & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Model}}} & \multicolumn{3}{c|}{\textbf{MAP}}                                                              & \multicolumn{3}{c}{\textbf{MRR}}                                                               \\ \cline{3-8} 
\multicolumn{1}{c|}{}                                       & \multicolumn{1}{c|}{}                                & \multicolumn{1}{c|}{\textbf{84\% data}}   & \multicolumn{2}{c|}{\textbf{100\% data}}           & \multicolumn{1}{c|}{\textbf{84\% data}}   & \multicolumn{2}{c}{\textbf{100\% data}}            \\ \cline{3-8} 
\multicolumn{1}{c|}{}                                       & \multicolumn{1}{c|}{}                                & \multicolumn{1}{c|}{\textbf{MAP$_{Best}$}}        & \multicolumn{1}{c|}{\textbf{MAP$_{2^{nd} Worst}$}} & \multicolumn{1}{c|}{\textbf{MAP$_{Worst}$}} & \multicolumn{1}{c|}{\textbf{MRR$_{Best}$}}        & \multicolumn{1}{c|}{\textbf{MRR$_{2^{nd} Worst}$}} & \multicolumn{1}{c}{\textbf{MRR$_{Worst}$}} \\ \hline
\multirow{8}{*}{AspectJ}                                    & RLocator                                             & \multicolumn{1}{c|}{\textbf{0.57}}        & \multicolumn{1}{c|}{0.47}          & \textbf{0.47} & \multicolumn{1}{c|}{\textbf{0.59}}        & \multicolumn{1}{c|}{0.5}           & 0.5           \\ \cline{2-8} 
                                                            & BugLocator                                           & \multicolumn{1}{c|}{0.33}                 & \multicolumn{1}{c|}{0.22}          & 0.22          & \multicolumn{1}{c|}{0.49}                 & \multicolumn{1}{c|}{0.42}          & 0.41          \\ \cline{2-8} 
                                                            & DeepLoc                                              & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{c|}{0.42}                          & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{c}{0.51}                           \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & CAST                                                 & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{0.42}                          & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{0.54}                           \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & KGBugLocator                                         & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{0.42}                          & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{\textbf{0.55}}                  \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & BL-GAN                                               & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{0.34}                          & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{-}                              \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & FBL-BERT                                             & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{0.08}                          & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{0.17}                           \\ \cline{2-8} 
                                                            & FLIM                                                 & \multicolumn{1}{c|}{0.41}                 & \multicolumn{1}{c|}{0.31}          & 0.31          & \multicolumn{1}{c|}{0.48}                 & \multicolumn{1}{c|}{0.41}          & 0.40          \\ \Xhline{3\arrayrulewidth}
\multirow{8}{*}{Birt}                                       & RLocator                                             & \multicolumn{1}{c|}{\textbf{0.47}}        & \multicolumn{1}{c|}{0.412}         & \textbf{0.41} & \multicolumn{1}{c|}{\textbf{0.49}}        & \multicolumn{1}{c|}{0.41}          & \textbf{0.4}  \\ \cline{2-8} 
                                                            & BugLocator                                           & \multicolumn{1}{c|}{0.30}                 & \multicolumn{1}{c|}{0.26}          & 0.25          & \multicolumn{1}{c|}{0.39}                 & \multicolumn{1}{c|}{0.28}          & 0.28          \\ \cline{2-8} 
                                                            & DeepLoc                                              & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{c|}{-}                             & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{c}{-}                              \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & CAST                                                 & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{-}                             & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{-}                              \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & KGBugLocator                                         & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{-}                             & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{-}                              \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & BL-GAN                                               & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{-}                             & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{-}                              \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & FBL-BERT                                             & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{-}                             & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{-}                              \\ \cline{2-8} 
                                                            & FLIM                                                 & \multicolumn{1}{c|}{0.30}                 & \multicolumn{1}{c|}{0.21}          & 0.24          & \multicolumn{1}{c|}{0.35}                 & \multicolumn{1}{c|}{0.26}          & 0.26          \\ \Xhline{3\arrayrulewidth}
\multirow{8}{*}{Eclipse Platform UI}                        & RLocator                                             & \multicolumn{1}{c|}{\textbf{0.55}}        & \multicolumn{1}{c|}{0.43}          & 0.43          & \multicolumn{1}{c|}{\textbf{0.59}}        & \multicolumn{1}{c|}{0.52}          & 0.51          \\ \cline{2-8} 
                                                            & BugLocator                                           & \multicolumn{1}{c|}{0.29}                 & \multicolumn{1}{c|}{0.23}          & 0.23          & \multicolumn{1}{c|}{0.38}                 & \multicolumn{1}{c|}{0.30}          & 0.30          \\ \cline{2-8} 
                                                            & DeepLoc                                              & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{c|}{0.43}                          & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{c}{\textbf{0.53}}                  \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & CAST                                                 & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{-}                             & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{-}                              \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & KGBugLocator                                         & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{-}                             & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{-}                              \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & BL-GAN                                               & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{0.32}                          & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{-}                              \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & FBL-BERT                                             & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{-}                             & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{-}                              \\ \cline{2-8} 
                                                            & FLIM                                                 & \multicolumn{1}{c|}{0.52}                 & \multicolumn{1}{c|}{0.48}          & \textbf{0.47} & \multicolumn{1}{c|}{0.57}                 & \multicolumn{1}{c|}{0.52}          & 0.51          \\ \Xhline{3\arrayrulewidth}
\multirow{8}{*}{JDT}                                        & RLocator                                             & \multicolumn{1}{c|}{\textbf{0.51}}        & \multicolumn{1}{c|}{0.44}          & 0.44          & \multicolumn{1}{c|}{\textbf{0.53}}        & \multicolumn{1}{c|}{0.47}          & 0.47          \\ \cline{2-8} 
                                                            & BugLocator                                           & \multicolumn{1}{c|}{0.22}                 & \multicolumn{1}{c|}{0.14}          & 0.14          & \multicolumn{1}{c|}{0.31}                 & \multicolumn{1}{c|}{0.18}          & 0.18          \\ \cline{2-8} 
                                                            & DeepLoc                                              & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{c|}{0.44}                          & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{c}{\textbf{0.53}}                  \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & CAST                                                 & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{\textbf{0.47}}                 & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{0.39}                           \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & KGBugLocator                                         & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{0.4}                           & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{0.47}                           \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & BL-GAN                                               & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{0.32}                          & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{-}                              \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & FBL-BERT                                             & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{0.06}                          & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{0.36}                           \\ \cline{2-8} 
                                                            & FLIM                                                 & \multicolumn{1}{c|}{0.50}                 & \multicolumn{1}{c|}{0.41}          & 0.40          & \multicolumn{1}{c|}{\textbf{0.53}}                 & \multicolumn{1}{c|}{0.49}          & 0.48          \\ \Xhline{3\arrayrulewidth}
\multirow{8}{*}{SWT}                                        & RLocator                                             & \multicolumn{1}{c|}{\textbf{0.48}}        & \multicolumn{1}{c|}{0.44}          & \textbf{0.44} & \multicolumn{1}{c|}{0.51}                 & \multicolumn{1}{c|}{0.45}          & 0.42          \\ \cline{2-8} 
                                                            & BugLocator                                           & \multicolumn{1}{c|}{0.47}                 & \multicolumn{1}{c|}{0.42}          & 0.41          & \multicolumn{1}{c|}{0.49}                 & \multicolumn{1}{c|}{0.45}          & 0.45          \\ \cline{2-8} 
                                                            & DeepLoc                                              & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{c|}{0.40}                          & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{c}{0.49}                           \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & CAST                                                 & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{0.42}                          & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{0.50}                           \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & KGBugLocator                                         & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{0.43}                          & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{\textbf{0.51}}                  \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & BL-GAN                                               & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{-}                             & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{-}                              \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & FBL-BERT                                             & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{0.12}                          & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{\textbf{0.51}}                  \\ \cline{2-8} 
                                                            & FLIM                                                 & \multicolumn{1}{c|}{0.47}                 & \multicolumn{1}{c|}{0.41}          & 0.40          & \multicolumn{1}{c|}{\textbf{0.52}}        & \multicolumn{1}{c|}{0.45}          & 0.43          \\ \Xhline{3\arrayrulewidth}
\multirow{8}{*}{Tomcat}                                     & RLocator                                             & \multicolumn{1}{c|}{\textbf{0.59}}        & \multicolumn{1}{c|}{0.52}          & 0.52          & \multicolumn{1}{c|}{\textbf{0.62}}        & \multicolumn{1}{c|}{0.5}           & 0.5           \\ \cline{2-8} 
                                                            & BugLocator                                           & \multicolumn{1}{c|}{0.31}                 & \multicolumn{1}{c|}{0.24}          & 0.22          & \multicolumn{1}{c|}{0.37}                 & \multicolumn{1}{c|}{0.31}          & 0.31          \\ \cline{2-8} 
                                                            & DeepLoc                                              & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{c|}{\textbf{0.56}}                 & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{c}{\textbf{0.62}}                  \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & CAST                                                 & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{0.55}                          & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{0.61}                           \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & KGBugLocator                                         & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{\textbf{0.56}}                 & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{\textbf{0.62}}                  \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & BL-GAN                                               & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{0.45}                          & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{-}                              \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                                            & FBL-BERT                                             & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c|}{0.13}                          & \multicolumn{1}{c|}{}                     & \multicolumn{2}{c}{0.43}                           \\ \cline{2-8} 
                                                            & FLIM                                                 & \multicolumn{1}{r|}{0.54}                 & \multicolumn{1}{c|}{0.47}          & 0.45          & \multicolumn{1}{c|}{0.61}                 & \multicolumn{1}{c|}{0.53}          & 0.53          \\ \hline
\end{tabular}
\label{table:result}
\end{table*}

==> Tables/result4.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[tb!]
\centering
\caption{RLocator performance.}
\begin{tabular}{c|c|ccl|ccl}
\hline
\multirow{3}{*}{\textbf{Project Name}} & \multirow{3}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{MAP}}                                                                                    & \multicolumn{3}{c}{\textbf{MRR}}                                                                                    \\ \cline{3-8} 
                                       &                                 & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{90\% data}}} & \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{100\% data}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{90\% data}}} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{100\% data}}} \\
                                       &                                 & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{}                                     & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{}                                     \\ \hline
\multirow{8}{*}{AspectJ}               & RLocator                        & \multicolumn{1}{c|}{\textbf{0.56}}                       & \multicolumn{2}{c|}{\textbf{0.46}}                        & \multicolumn{1}{c|}{\textbf{0.59}}                       & \multicolumn{2}{c}{0.50}                                 \\ \cline{2-8} 
                                       & BugLocator                      & \multicolumn{1}{c|}{0.33}                                & \multicolumn{2}{c|}{0.31}                                 & \multicolumn{1}{c|}{0.49}                                & \multicolumn{2}{c}{0.48}                                 \\ \cline{2-8} 
                                       & FLIM                            & \multicolumn{1}{c|}{0.41}                                & \multicolumn{2}{c|}{0.35}                                 & \multicolumn{1}{c|}{0.47}                                & \multicolumn{2}{c}{0.45}                                 \\ \cline{2-8} 
                                       & DeepLoc                         & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}}                & \multicolumn{2}{c|}{0.42}                                 & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}}                & \multicolumn{2}{c}{0.51}                                 \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & CAST                            & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{0.42}                                 & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{0.54}                                 \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & KGBugLocator                    & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{0.42}                                 & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{\textbf{0.55}}                        \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & BL-GAN                          & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{0.34}                                 & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{-}                                    \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & FBL-BERT                        & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{0.08}                                 & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{0.17}                                 \\ \hline
\multirow{8}{*}{Birt}                  & RLocator                        & \multicolumn{1}{c|}{\textbf{0.47}}                       & \multicolumn{2}{c|}{\textbf{0.38}}                        & \multicolumn{1}{c|}{\textbf{0.49}}                       & \multicolumn{2}{c}{\textbf{0.41}}                        \\ \cline{2-8} 
                                       & BugLocator                      & \multicolumn{1}{c|}{0.30}                                & \multicolumn{2}{c|}{0.30}                                 & \multicolumn{1}{c|}{0.39}                                & \multicolumn{2}{c}{0.38}                                 \\ \cline{2-8} 
                                       & FLIM                            & \multicolumn{1}{c|}{0.29}                                & \multicolumn{2}{c|}{0.25}                                 & \multicolumn{1}{c|}{0.31}                                & \multicolumn{2}{c}{0.28}                                 \\ \cline{2-8} 
                                       & DeepLoc                         & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}}                & \multicolumn{2}{c|}{-}                                    & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}}                & \multicolumn{2}{c}{-}                                    \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & CAST                            & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{-}                                    & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{-}                                    \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & KGBugLocator                    & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{-}                                    & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{-}                                    \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & BL-GAN                          & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{-}                                    & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{-}                                    \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & FBL-BERT                        & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{-}                                    & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{-}                                    \\ \hline
\multirow{8}{*}{Eclipse Platform UI}   & RLocator                        & \multicolumn{1}{c|}{\textbf{0.54}}                       & \multicolumn{2}{c|}{0.42}                                 & \multicolumn{1}{c|}{\textbf{0.59}}                       & \multicolumn{2}{c}{0.50}                                 \\ \cline{2-8} 
                                       & BugLocator                      & \multicolumn{1}{c|}{0.29}                                & \multicolumn{2}{c|}{0.30}                                 & \multicolumn{1}{c|}{0.38}                                & \multicolumn{2}{c}{0.35}                                 \\ \cline{2-8} 
                                       & FLIM                            & \multicolumn{1}{c|}{0.51}                                & \multicolumn{2}{c|}{\textbf{0.48}}                        & \multicolumn{1}{c|}{0.52}                                & \multicolumn{2}{c}{\textbf{0.53}}                        \\ \cline{2-8} 
                                       & DeepLoc                         & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}}                & \multicolumn{2}{c|}{0.43}                                 & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}}                & \multicolumn{2}{c}{\textbf{0.53}}                        \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & CAST                            & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{-}                                    & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{-}                                    \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & KGBugLocator                    & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{-}                                    & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{-}                                    \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & BL-GAN                          & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{0.32}                                 & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{-}                                    \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & FBL-BERT                        & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{-}                                    & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{-}                                    \\ \hline
\multirow{8}{*}{JDT}                   & RLocator                        & \multicolumn{1}{c|}{\textbf{0.51}}                       & \multicolumn{2}{c|}{0.44}                                 & \multicolumn{1}{c|}{\textbf{0.53}}                       & \multicolumn{2}{c}{0.45}                                 \\ \cline{2-8} 
                                       & BugLocator                      & \multicolumn{1}{c|}{0.22}                                & \multicolumn{2}{c|}{0.20}                                 & \multicolumn{1}{c|}{0.31}                                & \multicolumn{2}{c}{0.28}                                 \\ \cline{2-8} 
                                       & FLIM                            & \multicolumn{1}{c|}{0.42}                                & \multicolumn{2}{c|}{0.41}                                 & \multicolumn{1}{c|}{0.51}                                & \multicolumn{2}{c}{0.49}                                 \\ \cline{2-8} 
                                       & DeepLoc                         & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}}                & \multicolumn{2}{c|}{0.44}                                 & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}}                & \multicolumn{2}{c}{\textbf{0.53}}                        \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & CAST                            & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{\textbf{0.47}}                        & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{0.39}                                 \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & KGBugLocator                    & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{0.4}                                  & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{0.47}                                 \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & BL-GAN                          & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{0.32}                                 & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{-}                                    \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & FBL-BERT                        & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{0.06}                                 & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{0.36}                                 \\ \hline
\multirow{8}{*}{SWT}                   & RLocator                        & \multicolumn{1}{c|}{\textbf{0.48}}                       & \multicolumn{2}{c|}{0.42}                                 & \multicolumn{1}{c|}{\textbf{0.51}}                       & \multicolumn{2}{c}{0.44}                                 \\ \cline{2-8} 
                                       & BugLocator                      & \multicolumn{1}{c|}{0.47}                                & \multicolumn{2}{c|}{\textbf{0.45}}                        & \multicolumn{1}{c|}{0.49}                                & \multicolumn{2}{c}{0.43}                                 \\ \cline{2-8} 
                                       & FLIM                            & \multicolumn{1}{c|}{0.43}                                & \multicolumn{2}{c|}{0.43}                                 & \multicolumn{1}{c|}{0.48}                                & \multicolumn{2}{c}{0.50}                                 \\ \cline{2-8} 
                                       & DeepLoc                         & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}}                & \multicolumn{2}{c|}{0.40}                                 & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}}                & \multicolumn{2}{c}{0.49}                                 \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & CAST                            & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{0.42}                                 & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{0.50}                                 \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & KGBugLocator                    & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{0.43}                                 & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{\textbf{0.51}}                        \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & BL-GAN                          & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{-}                                    & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{-}                                    \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & FBL-BERT                        & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{0.12}                                 & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{\textbf{0.51}}                        \\ \hline
\multirow{8}{*}{Tomcat}                & RLocator                        & \multicolumn{1}{c|}{\textbf{0.59}}                       & \multicolumn{2}{c|}{0.47}                                 & \multicolumn{1}{c|}{\textbf{0.62}}                       & \multicolumn{2}{c}{0.51}                                 \\ \cline{2-8} 
                                       & BugLocator                      & \multicolumn{1}{c|}{0.31}                                & \multicolumn{2}{c|}{0.27}                                 & \multicolumn{1}{c|}{0.37}                                & \multicolumn{2}{c}{0.35}                                 \\ \cline{2-8} 
                                       & FLIM                            & \multicolumn{1}{c|}{0.52}                                & \multicolumn{2}{c|}{0.47}                                 & \multicolumn{1}{c|}{0.59}                                & \multicolumn{2}{c}{0.60}                                 \\ \cline{2-8} 
                                       & DeepLoc                         & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}}                & \multicolumn{2}{c|}{\textbf{0.56}}                        & \multicolumn{1}{c|}{\multirow{5}{*}{N/A}}                & \multicolumn{2}{c}{\textbf{0.62}}                        \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & CAST                            & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{0.55}                                 & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{0.61}                                 \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & KGBugLocator                    & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{\textbf{0.56}}                        & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{\textbf{0.62}}                        \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & BL-GAN                          & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{0.45}                                 & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{-}                                    \\ \cline{2-2} \cline{4-5} \cline{7-8} 
                                       & FBL-BERT                        & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c|}{0.13}                                 & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{c}{0.43}                                 \\ \hline
\end{tabular}
\label{table:result}
\end{table*}

==> Tables/result_1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{|l|l|rrr|rrr|}
\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{Project Name}}} & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Model}}} & \multicolumn{3}{c|}{\textbf{MAP}}                                                                                 & \multicolumn{3}{c|}{\textbf{MRR}}                                                                                 \\ \cline{3-8} 
\multicolumn{1}{|c|}{}                                       & \multicolumn{1}{c|}{}                                & \multicolumn{1}{c|}{\textbf{85\% data}} & \multicolumn{2}{c|}{\textbf{100\% data}}                                & \multicolumn{1}{c|}{\textbf{85\% data}} & \multicolumn{2}{c|}{\textbf{100\% data}}                                \\ \cline{3-8} 
\multicolumn{1}{|c|}{}                                       & \multicolumn{1}{c|}{}                                & \multicolumn{1}{c|}{\textbf{MAP1}}      & \multicolumn{1}{c|}{\textbf{MAP2}} & \multicolumn{1}{c|}{\textbf{MAP3}} & \multicolumn{1}{c|}{\textbf{MRR1}}      & \multicolumn{1}{c|}{\textbf{MRR2}} & \multicolumn{1}{c|}{\textbf{MRR3}} \\ \hline
\multirow{8}{*}{AspectJ}                                     & RLocator                                             & \multicolumn{1}{r|}{\textbf{0.57}}      & \multicolumn{1}{r|}{0.47}          & 0.47                               & \multicolumn{1}{r|}{\textbf{0.59}}      & \multicolumn{1}{r|}{0.5}           & 0.5                                \\ \cline{2-8} 
                                                             & BugLocator                                           & \multicolumn{1}{r|}{0.33}               & \multicolumn{1}{r|}{0.22}          & 0.22                               & \multicolumn{1}{r|}{0.49}               & \multicolumn{1}{r|}{0.42}          & 0.41                               \\ \cline{2-8} 
                                                             & DeepLoc                                              & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.42}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.51}                                               \\ \cline{2-8} 
                                                             & CAST                                                 & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.42}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.54}                                               \\ \cline{2-8} 
                                                             & KGBugLocator                                         & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.42}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.55}                                               \\ \cline{2-8} 
                                                             & BL-GAN                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.34}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  \\ \cline{2-8} 
                                                             & FBL-BERT                                             & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.08}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.17}                                               \\ \cline{2-8} 
                                                             & FLIM                                                 & \multicolumn{1}{r|}{0.41}               & \multicolumn{1}{r|}{0.31}          & 0.31                               & \multicolumn{1}{r|}{0.48}               & \multicolumn{1}{r|}{0.41}          & 0.40                               \\ \hline
\multirow{8}{*}{Birt}                                        & RLocator                                             & \multicolumn{1}{r|}{\textbf{0.47}}      & \multicolumn{1}{r|}{0.412}         & 0.41                               & \multicolumn{1}{r|}{\textbf{0.49}}      & \multicolumn{1}{r|}{0.41}          & 0.4                                \\ \cline{2-8} 
                                                             & BugLocator                                           & \multicolumn{1}{r|}{0.30}               & \multicolumn{1}{r|}{0.26}          & 0.25                               & \multicolumn{1}{r|}{0.39}               & \multicolumn{1}{r|}{0.28}          & 0.28                               \\ \cline{2-8} 
                                                             & DeepLoc                                              & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  \\ \cline{2-8} 
                                                             & CAST                                                 & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  \\ \cline{2-8} 
                                                             & KGBugLocator                                         & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  \\ \cline{2-8} 
                                                             & BL-GAN                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  \\ \cline{2-8} 
                                                             & FBL-BERT                                             & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  \\ \cline{2-8} 
                                                             & FLIM                                                 & \multicolumn{1}{r|}{0.30}               & \multicolumn{1}{r|}{0.21}          & 0.24                               & \multicolumn{1}{r|}{0.35}               & \multicolumn{1}{r|}{0.26}          & 0.26                               \\ \hline
\multirow{8}{*}{Eclipse Platform UI}                         & RLocator                                             & \multicolumn{1}{r|}{\textbf{0.55}}      & \multicolumn{1}{r|}{0.43}          & 0.43                               & \multicolumn{1}{r|}{\textbf{0.59}}      & \multicolumn{1}{r|}{0.52}          & 0.51                               \\ \cline{2-8} 
                                                             & BugLocator                                           & \multicolumn{1}{r|}{0.29}               & \multicolumn{1}{r|}{0.23}          & 0.23                               & \multicolumn{1}{r|}{0.38}               & \multicolumn{1}{r|}{0.30}          & 0.30                               \\ \cline{2-8} 
                                                             & DeepLoc                                              & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.43}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.53}                                               \\ \cline{2-8} 
                                                             & CAST                                                 & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  \\ \cline{2-8} 
                                                             & KGBugLocator                                         & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  \\ \cline{2-8} 
                                                             & BL-GAN                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.32}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  \\ \cline{2-8} 
                                                             & FBL-BERT                                             & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  \\ \cline{2-8} 
                                                             & FLIM                                                 & \multicolumn{1}{r|}{0.52}               & \multicolumn{1}{r|}{0.48}          & 0.47                               & \multicolumn{1}{r|}{0.57}               & \multicolumn{1}{r|}{0.52}          & 0.51                               \\ \hline
\multirow{8}{*}{JDT}                                         & RLocator                                             & \multicolumn{1}{r|}{\textbf{0.51}}      & \multicolumn{1}{r|}{0.44}          & 0.44                               & \multicolumn{1}{r|}{\textbf{0.53}}      & \multicolumn{1}{r|}{0.47}          & 0.47                               \\ \cline{2-8} 
                                                             & BugLocator                                           & \multicolumn{1}{r|}{0.22}               & \multicolumn{1}{r|}{0.14}          & 0.14                               & \multicolumn{1}{r|}{0.31}               & \multicolumn{1}{r|}{0.18}          & 0.18                               \\ \cline{2-8} 
                                                             & DeepLoc                                              & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.44}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{\textbf{0.53}}                                      \\ \cline{2-8} 
                                                             & CAST                                                 & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.47}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.39}                                               \\ \cline{2-8} 
                                                             & KGBugLocator                                         & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.4}                                                & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.47}                                               \\ \cline{2-8} 
                                                             & BL-GAN                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.32}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  \\ \cline{2-8} 
                                                             & FBL-BERT                                             & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.06}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.36}                                               \\ \cline{2-8} 
                                                             & FLIM                                                 & \multicolumn{1}{r|}{0.50}               & \multicolumn{1}{r|}{0.41}          & 0.40                               & \multicolumn{1}{r|}{0.53}               & \multicolumn{1}{r|}{0.49}          & 0.48                               \\ \hline
\multirow{8}{*}{SWT}                                         & RLocator                                             & \multicolumn{1}{r|}{\textbf{0.48}}      & \multicolumn{1}{r|}{0.44}          & 0.44                               & \multicolumn{1}{r|}{0.51}               & \multicolumn{1}{r|}{0.45}          & 0.42                               \\ \cline{2-8} 
                                                             & BugLocator                                           & \multicolumn{1}{r|}{0.47}               & \multicolumn{1}{r|}{0.42}          & 0.41                               & \multicolumn{1}{r|}{0.49}               & \multicolumn{1}{r|}{0.45}          & 0.45                               \\ \cline{2-8} 
                                                             & DeepLoc                                              & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.40}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.49}                                               \\ \cline{2-8} 
                                                             & CAST                                                 & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.42}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.50}                                               \\ \cline{2-8} 
                                                             & KGBugLocator                                         & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.43}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.51}                                               \\ \cline{2-8} 
                                                             & BL-GAN                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  \\ \cline{2-8} 
                                                             & FBL-BERT                                             & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.12}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.51}                                               \\ \cline{2-8} 
                                                             & FLIM                                                 & \multicolumn{1}{r|}{0.47}               & \multicolumn{1}{r|}{0.41}          & 0.40                               & \multicolumn{1}{r|}{\textbf{0.52}}      & \multicolumn{1}{r|}{0.45}          & 0.43                               \\ \hline
\multirow{8}{*}{Tomcat}                                      & RLocator                                             & \multicolumn{1}{r|}{\textbf{0.59}}      & \multicolumn{1}{r|}{0.52}          & 0.52                               & \multicolumn{1}{r|}{\textbf{0.62}}      & \multicolumn{1}{r|}{0.5}           & 0.5                                \\ \cline{2-8} 
                                                             & BugLocator                                           & \multicolumn{1}{r|}{0.31}               & \multicolumn{1}{r|}{0.24}          & 0.22                               & \multicolumn{1}{r|}{0.37}               & \multicolumn{1}{r|}{0.31}          & 0.31                               \\ \cline{2-8} 
                                                             & DeepLoc                                              & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.56}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{\textbf{0.62}}                                      \\ \cline{2-8} 
                                                             & CAST                                                 & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.55}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.61}                                               \\ \cline{2-8} 
                                                             & KGBugLocator                                         & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.56}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{\textbf{0.62}}                                      \\ \cline{2-8} 
                                                             & BL-GAN                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.45}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{-}                                                  \\ \cline{2-8} 
                                                             & FBL-BERT                                             & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.13}                                               & \multicolumn{1}{r|}{N/A}                & \multicolumn{2}{r|}{0.43}                                               \\ \cline{2-8} 
                                                             & FLIM                                                 & \multicolumn{1}{r|}{0.54}               & \multicolumn{1}{r|}{0.47}          & 0.45                               & \multicolumn{1}{r|}{0.61}               & \multicolumn{1}{r|}{0.53}          & 0.53                               \\ \hline
\end{tabular}
\end{table*}

==> Tables/result_2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{l|l|rrr|rrr}
\toprule
\multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Project Name}}} & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Model}}} & \multicolumn{3}{c|}{\textbf{MAP}}                                                                                   & \multicolumn{3}{c}{\textbf{MRR}}                                                                                   \\ \cmidrule{3-8} 
\multicolumn{1}{c|}{}                                       & \multicolumn{1}{c|}{}                                & \multicolumn{1}{c|}{\textbf{85\% data}}   & \multicolumn{2}{c|}{\textbf{100\% data}}                                & \multicolumn{1}{c|}{\textbf{85\% data}}   & \multicolumn{2}{c}{\textbf{100\% data}}                                \\ \cmidrule{3-8} 
\multicolumn{1}{c|}{}                                       & \multicolumn{1}{c|}{}                                & \multicolumn{1}{c|}{\textbf{MAP$_{Best}$}}        & \multicolumn{1}{c|}{\textbf{MAP$_{2^{nd} Worst}$}} & \multicolumn{1}{c|}{\textbf{MAP$_{Worst}$}} & \multicolumn{1}{c|}{\textbf{MRR$_{Best}$}}        & \multicolumn{1}{c|}{\textbf{MRR$_{2^{nd} Worst}$}} & \multicolumn{1}{c|}{\textbf{MRR$_{Worst}$}} \\ \midrule
\multirow{8}{*}{AspectJ}                                    & RLocator                                             & \multicolumn{1}{r|}{\textbf{0.57}}        & \multicolumn{1}{r|}{0.47}          & 0.47                               & \multicolumn{1}{r|}{\textbf{0.59}}        & \multicolumn{1}{r|}{0.5}           & 0.5                               \\ \cmidrule{2-8} 
                                                            & BugLocator                                           & \multicolumn{1}{r|}{0.33}                 & \multicolumn{1}{r|}{0.22}          & 0.22                               & \multicolumn{1}{r|}{0.49}                 & \multicolumn{1}{r|}{0.42}          & 0.41                              \\ \cmidrule{2-8} 
                                                            & DeepLoc                                              & \multicolumn{1}{r|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{r|}{0.42}                                               & \multicolumn{1}{r|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{r}{0.51}                                               \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & CAST                                                 & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{0.42}                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{0.54}                                               \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & KGBugLocator                                         & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{0.42}                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{0.55}                                               \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & BL-GAN                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{0.34}                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{-}                                                  \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & FBL-BERT                                             & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{0.08}                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{0.17}                                               \\ \cmidrule{2-8} 
                                                            & FLIM                                                 & \multicolumn{1}{r|}{0.41}                 & \multicolumn{1}{r|}{0.31}          & 0.31                               & \multicolumn{1}{r|}{0.48}                 & \multicolumn{1}{r|}{0.41}          & 0.40                              \\ \midrule
\multirow{8}{*}{Birt}                                       & RLocator                                             & \multicolumn{1}{r|}{\textbf{0.47}}        & \multicolumn{1}{r|}{0.412}         & 0.41                               & \multicolumn{1}{r|}{\textbf{0.49}}        & \multicolumn{1}{r|}{0.41}          & 0.4                               \\ \cmidrule{2-8} 
                                                            & BugLocator                                           & \multicolumn{1}{r|}{0.30}                 & \multicolumn{1}{r|}{0.26}          & 0.25                               & \multicolumn{1}{r|}{0.39}                 & \multicolumn{1}{r|}{0.28}          & 0.28                              \\ \cmidrule{2-8} 
                                                            & DeepLoc                                              & \multicolumn{1}{r|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{r|}{-}                                                  & \multicolumn{1}{r|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{r}{-}                                                  \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & CAST                                                 & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{-}                                                  & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{-}                                                  \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & KGBugLocator                                         & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{-}                                                  & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{-}                                                  \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & BL-GAN                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{-}                                                  & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{-}                                                  \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & FBL-BERT                                             & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{-}                                                  & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{-}                                                  \\ \cmidrule{2-8} 
                                                            & FLIM                                                 & \multicolumn{1}{r|}{0.30}                 & \multicolumn{1}{r|}{0.21}          & 0.24                               & \multicolumn{1}{r|}{0.35}                 & \multicolumn{1}{r|}{0.26}          & 0.26                              \\ \midrule
\multirow{8}{*}{Eclipse Platform UI}                        & RLocator                                             & \multicolumn{1}{r|}{\textbf{0.55}}        & \multicolumn{1}{r|}{0.43}          & 0.43                               & \multicolumn{1}{r|}{\textbf{0.59}}        & \multicolumn{1}{r|}{0.52}          & 0.51                              \\ \cmidrule{2-8} 
                                                            & BugLocator                                           & \multicolumn{1}{r|}{0.29}                 & \multicolumn{1}{r|}{0.23}          & 0.23                               & \multicolumn{1}{r|}{0.38}                 & \multicolumn{1}{r|}{0.30}          & 0.30                              \\ \cmidrule{2-8} 
                                                            & DeepLoc                                              & \multicolumn{1}{r|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{r|}{0.43}                                               & \multicolumn{1}{r|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{r}{0.53}                                               \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & CAST                                                 & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{-}                                                  & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{-}                                                  \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & KGBugLocator                                         & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{-}                                                  & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{-}                                                  \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & BL-GAN                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{0.32}                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{-}                                                  \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & FBL-BERT                                             & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{-}                                                  & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{-}                                                  \\ \cmidrule{2-8} 
                                                            & FLIM                                                 & \multicolumn{1}{r|}{0.52}                 & \multicolumn{1}{r|}{0.48}          & 0.47                               & \multicolumn{1}{r|}{0.57}                 & \multicolumn{1}{r|}{0.52}          & 0.51                              \\ \midrule
\multirow{8}{*}{JDT}                                        & RLocator                                             & \multicolumn{1}{r|}{\textbf{0.51}}        & \multicolumn{1}{r|}{0.44}          & 0.44                               & \multicolumn{1}{r|}{\textbf{0.53}}        & \multicolumn{1}{r|}{0.47}          & 0.47                              \\ \cmidrule{2-8} 
                                                            & BugLocator                                           & \multicolumn{1}{r|}{0.22}                 & \multicolumn{1}{r|}{0.14}          & 0.14                               & \multicolumn{1}{r|}{0.31}                 & \multicolumn{1}{r|}{0.18}          & 0.18                              \\ \cmidrule{2-8} 
                                                            & DeepLoc                                              & \multicolumn{1}{r|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{r|}{0.44}                                               & \multicolumn{1}{r|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{r}{\textbf{0.53}}                                      \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & CAST                                                 & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{0.47}                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{0.39}                                               \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & KGBugLocator                                         & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{0.4}                                                & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{0.47}                                               \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & BL-GAN                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{0.32}                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{-}                                                  \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & FBL-BERT                                             & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{0.06}                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{0.36}                                               \\ \cmidrule{2-8} 
                                                            & FLIM                                                 & \multicolumn{1}{r|}{0.50}                 & \multicolumn{1}{r|}{0.41}          & 0.40                               & \multicolumn{1}{r|}{0.53}                 & \multicolumn{1}{r|}{0.49}          & 0.48                              \\ \midrule
\multirow{8}{*}{SWT}                                        & RLocator                                             & \multicolumn{1}{r|}{\textbf{0.48}}        & \multicolumn{1}{r|}{0.44}          & 0.44                               & \multicolumn{1}{r|}{0.51}                 & \multicolumn{1}{r|}{0.45}          & 0.42                              \\ \cmidrule{2-8} 
                                                            & BugLocator                                           & \multicolumn{1}{r|}{0.47}                 & \multicolumn{1}{r|}{0.42}          & 0.41                               & \multicolumn{1}{r|}{0.49}                 & \multicolumn{1}{r|}{0.45}          & 0.45                              \\ \cmidrule{2-8} 
                                                            & DeepLoc                                              & \multicolumn{1}{r|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{r|}{0.40}                                               & \multicolumn{1}{r|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{r}{0.49}                                               \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & CAST                                                 & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{0.42}                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{0.50}                                               \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & KGBugLocator                                         & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{0.43}                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{0.51}                                               \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & BL-GAN                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{-}                                                  & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{-}                                                  \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & FBL-BERT                                             & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{0.12}                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{0.51}                                               \\ \cmidrule{2-8} 
                                                            & FLIM                                                 & \multicolumn{1}{r|}{0.47}                 & \multicolumn{1}{r|}{0.41}          & 0.40                               & \multicolumn{1}{r|}{\textbf{0.52}}        & \multicolumn{1}{r|}{0.45}          & 0.43                              \\ \midrule
\multirow{8}{*}{Tomcat}                                     & RLocator                                             & \multicolumn{1}{r|}{\textbf{0.59}}        & \multicolumn{1}{r|}{0.52}          & 0.52                               & \multicolumn{1}{r|}{\textbf{0.62}}        & \multicolumn{1}{r|}{0.5}           & 0.5                               \\ \cmidrule{2-8} 
                                                            & BugLocator                                           & \multicolumn{1}{r|}{0.31}                 & \multicolumn{1}{r|}{0.24}          & 0.22                               & \multicolumn{1}{r|}{0.37}                 & \multicolumn{1}{r|}{0.31}          & 0.31                              \\ \cmidrule{2-8} 
                                                            & DeepLoc                                              & \multicolumn{1}{r|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{r|}{0.56}                                               & \multicolumn{1}{r|}{\multirow{5}{*}{N/A}} & \multicolumn{2}{r}{\textbf{0.62}}                                      \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & CAST                                                 & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{0.55}                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{0.61}                                               \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & KGBugLocator                                         & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{0.56}                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{\textbf{0.62}}                                      \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & BL-GAN                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{0.45}                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{-}                                                  \\ \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} 
                                                            & FBL-BERT                                             & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r|}{0.13}                                               & \multicolumn{1}{r|}{}                     & \multicolumn{2}{r}{0.43}                                               \\ \cmidrule{2-8} 
                                                            & FLIM                                                 & \multicolumn{1}{r|}{0.54}                 & \multicolumn{1}{r|}{0.47}          & 0.45                               & \multicolumn{1}{r|}{0.61}                 & \multicolumn{1}{r|}{0.53}          & 0.53                              \\ \bottomrule
\end{tabular}
\end{table*}

==> Tables/result_table1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{RLocator performance.}
\begin{tabular}{l|l|rr|rr|rr|rr|rr}
\hline
\multirow{2}{*}{\textbf{Project}}    & \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{r|}{\textbf{Top 1}}                 & \multicolumn{2}{r|}{\textbf{Top 5}}                 & \multicolumn{2}{r|}{\textbf{Top 10}}                & \multicolumn{2}{r|}{\textbf{MAP}}                   & \multicolumn{2}{r}{\textbf{MRR}}                   \\ \cline{3-12} 
                                     &                                 & \multicolumn{1}{r|}{\textbf{91\%}} & \textbf{100\%} & \multicolumn{1}{r|}{\textbf{91\%}} & \textbf{100\%} & \multicolumn{1}{r|}{\textbf{91\%}} & \textbf{100\%} & \multicolumn{1}{r|}{\textbf{91\%}} & \textbf{100\%} & \multicolumn{1}{r|}{\textbf{91\%}} & \textbf{100\%} \\ \hline
\multirow{3}{*}{AspectJ}             & RLocator                        & \multicolumn{1}{r|}{0.46}          & \textbf{0.40}  & \multicolumn{1}{r|}{\textbf{0.69}} & 0.63           & \multicolumn{1}{r|}{\textbf{0.75}} & \textbf{0.70}  & \multicolumn{1}{r|}{\textbf{0.56}} & \textbf{0.46}  & \multicolumn{1}{r|}{\textbf{0.59}} & \textbf{0.50}  \\ \cline{2-12} 
                                     & BugLocator                      & \multicolumn{1}{r|}{0.36}          & 0.28           & \multicolumn{1}{r|}{0.50}          & 0.45           & \multicolumn{1}{r|}{0.56}          & 0.51           & \multicolumn{1}{r|}{0.33}          & 0.31           & \multicolumn{1}{r|}{0.49}          & 0.48           \\ \cline{2-12} 
                                     & FLIM                            & \multicolumn{1}{r|}{\textbf{0.51}} & 0.36           & \multicolumn{1}{r|}{0.65}          & 0.60           & \multicolumn{1}{r|}{0.72}          & 0.67           & \multicolumn{1}{r|}{0.41}          & 0.35           & \multicolumn{1}{r|}{0.47}          & 0.45           \\ \hline
\multirow{3}{*}{Birt}                & RLocator                        & \multicolumn{1}{r|}{\textbf{0.38}} & \textbf{0.25}  & \multicolumn{1}{r|}{\textbf{0.46}} & \textbf{0.41}  & \multicolumn{1}{r|}{\textbf{0.53}} & \textbf{0.48}  & \multicolumn{1}{r|}{\textbf{0.47}} & \textbf{0.38}  & \multicolumn{1}{r|}{\textbf{0.49}} & \textbf{0.41}  \\ \cline{2-12} 
                                     & BugLocator                      & \multicolumn{1}{r|}{0.28}          & 0.15           & \multicolumn{1}{r|}{0.27}          & 0.21           & \multicolumn{1}{r|}{0.34}          & 0.29           & \multicolumn{1}{r|}{0.30}          & 0.30           & \multicolumn{1}{r|}{0.39}          & 0.38           \\ \cline{2-12} 
                                     & FLIM                            & \multicolumn{1}{r|}{0.29}          & 0.18           & \multicolumn{1}{r|}{0.39}          & 0.34           & \multicolumn{1}{r|}{0.47}          & 0.42           & \multicolumn{1}{r|}{0.29}          & 0.25           & \multicolumn{1}{r|}{0.31}          & 0.28           \\ \hline
\multirow{3}{*}{Eclipse Platform UI} & RLocator                        & \multicolumn{1}{r|}{0.45}          & 0.37           & \multicolumn{1}{r|}{0.69}          & 0.63           & \multicolumn{1}{r|}{0.78}          & 0.73           & \multicolumn{1}{r|}{\textbf{0.54}} & 0.42           & \multicolumn{1}{r|}{\textbf{0.59}} & 0.50           \\ \cline{2-12} 
                                     & BugLocator                      & \multicolumn{1}{r|}{0.45}          & 0.33           & \multicolumn{1}{r|}{0.54}          & 0.49           & \multicolumn{1}{r|}{0.63}          & 0.58           & \multicolumn{1}{r|}{0.29}          & 0.30           & \multicolumn{1}{r|}{0.38}          & 0.35           \\ \cline{2-12} 
                                     & FLIM                            & \multicolumn{1}{r|}{\textbf{0.48}} & \textbf{0.41}  & \multicolumn{1}{r|}{\textbf{0.72}} & \textbf{0.67}  & \multicolumn{1}{r|}{\textbf{0.80}} & \textbf{0.75}  & \multicolumn{1}{r|}{0.51}          & \textbf{0.48}  & \multicolumn{1}{r|}{0.52}          & \textbf{0.53}  \\ \hline
\multirow{3}{*}{JDT}                 & RLocator                        & \multicolumn{1}{r|}{\textbf{0.44}} & 0.33           & \multicolumn{1}{r|}{\textbf{0.67}} & \textbf{0.61}  & \multicolumn{1}{r|}{0.78}          & 0.75           & \multicolumn{1}{r|}{\textbf{0.51}} & \textbf{0.44}  & \multicolumn{1}{r|}{\textbf{0.53}} & 0.45           \\ \cline{2-12} 
                                     & BugLocator                      & \multicolumn{1}{r|}{0.34}          & 0.21           & \multicolumn{1}{r|}{0.51}          & 0.45           & \multicolumn{1}{r|}{0.60}          & 0.55           & \multicolumn{1}{r|}{0.22}          & 0.20           & \multicolumn{1}{r|}{0.31}          & 0.28           \\ \cline{2-12} 
                                     & FLIM                            & \multicolumn{1}{r|}{0.40}          & \textbf{0.35}  & \multicolumn{1}{r|}{0.65}          & 0.60           & \multicolumn{1}{r|}{\textbf{0.82}} & \textbf{0.77}  & \multicolumn{1}{r|}{0.42}          & 0.41           & \multicolumn{1}{r|}{0.51}          & \textbf{0.49}  \\ \hline
\multirow{3}{*}{SWT}                 & RLocator                        & \multicolumn{1}{r|}{0.40}          & 0.30           & \multicolumn{1}{r|}{0.57}          & 0.51           & \multicolumn{1}{r|}{0.63}          & 0.58           & \multicolumn{1}{r|}{\textbf{0.48}} & 0.42           & \multicolumn{1}{r|}{\textbf{0.51}} & 0.44           \\ \cline{2-12} 
                                     & BugLocator                      & \multicolumn{1}{r|}{0.37}          & 0.25           & \multicolumn{1}{r|}{0.50}          & 0.45           & \multicolumn{1}{r|}{0.56}          & 0.51           & \multicolumn{1}{r|}{0.42}          & 0.40           & \multicolumn{1}{r|}{0.46}          & 0.43           \\ \cline{2-12} 
                                     & FLIM                            & \multicolumn{1}{r|}{\textbf{0.51}} & \textbf{0.37}  & \multicolumn{1}{r|}{\textbf{0.70}} & \textbf{0.65}  & \multicolumn{1}{r|}{\textbf{0.83}} & \textbf{0.78}  & \multicolumn{1}{r|}{0.43}          & \textbf{0.43}  & \multicolumn{1}{r|}{0.48}          & \textbf{0.50}  \\ \hline
\multirow{3}{*}{Tomcat}              & RLocator                        & \multicolumn{1}{r|}{0.46}          & 0.39           & \multicolumn{1}{r|}{0.61}          & 0.55           & \multicolumn{1}{r|}{0.73}          & 0.68           & \multicolumn{1}{r|}{\textbf{0.59}} & \textbf{0.47}  & \multicolumn{1}{r|}{\textbf{0.62}} & 0.51           \\ \cline{2-12} 
                                     & BugLocator                      & \multicolumn{1}{r|}{0.40}          & 0.29           & \multicolumn{1}{r|}{0.43}          & 0.38           & \multicolumn{1}{r|}{0.55}          & 0.50           & \multicolumn{1}{r|}{0.31}          & 0.27           & \multicolumn{1}{r|}{0.37}          & 0.35           \\ \cline{2-12} 
                                     & FLIM                            & \multicolumn{1}{r|}{\textbf{0.51}} & \textbf{0.42}  & \multicolumn{1}{r|}{\textbf{0.70}} & \textbf{0.65}  & \multicolumn{1}{r|}{\textbf{0.76}} & \textbf{0.71}  & \multicolumn{1}{r|}{0.52}          & \textbf{0.47}  & \multicolumn{1}{r|}{0.59}          & \textbf{0.60}  \\ \hline
\end{tabular}
\label{table:result}
\end{table*}



==> Tables/result_table2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[tb!]
\centering
\caption{Performance comparison of RLocator over 100\% data.}
\begin{tabular}{c|c|r|r|r|r|r}
\hline
\textbf{Project}                     & \textbf{Model} & \textbf{Top 1} & \textbf{Top 5} & \textbf{Top 10} & \textbf{MAP} & \textbf{MRR} \\ \hline
\multirow{5}{*}{AspectJ}             & RLocator       & 0.40           & 0.63           & 0.70            & 0.46         & 0.50         \\ \cline{2-7} 
                                     & DeepLoc        & 0.45           & 0.71           & 0.80            & 0.42         & 0.51         \\ \cline{2-7} 
                                     & CAST           & 0.50           & 0.76           & 0.83            & 0.42         & 0.54         \\ \cline{2-7} 
                                     & KGBugLocator   & 0.50           & 0.77           & 0.83            & 0.42         & 0.55         \\ \cline{2-7} 
                                     & BL-GAN         & 0.41           & 0.60           & 0.73            & 0.34         & -            \\ \hline
\multirow{5}{*}{Birt}                & RLocator       & 0.25           & 0.41           & 0.48            & 0.38         & 0.41         \\ \cline{2-7} 
                                     & DeepLoc        & -              & -              & -               & -            & -            \\ \cline{2-7} 
                                     & CAST           & -              & -              & -               & -            & -            \\ \cline{2-7} 
                                     & KGBugLocator   & -              & -              & -               & -            & -            \\ \cline{2-7} 
                                     & BL-GAN         & -              & -              & -               & -            & -            \\ \hline
\multirow{5}{*}{Eclipse Platform UI} & RLocator       & 0.37           & 0.63           & 0.73            & 0.42         & 0.50         \\ \cline{2-7} 
                                     & DeepLoc        & 0.45           & 0.70           & 0.79            & 0.43         & 0.53         \\ \cline{2-7} 
                                     & CAST           & -              & -              & -               & -            & -            \\ \cline{2-7} 
                                     & KGBugLocator   & -              & -              & -               & -            & -            \\ \cline{2-7} 
                                     & BL-GAN         & 0.34           & 0.50           & 0.64            & -            & -            \\ \hline
\multirow{5}{*}{JDT}                 & RLocator       & 0.33           & 0.61           & 0.75            & 0.44         & 0.45         \\ \cline{2-7} 
                                     & DeepLoc        & 0.43           & 0.65           & 0.77            & 0.44         & 0.53         \\ \cline{2-7} 
                                     & CAST           & 0.43           & 0.68           & 0.75            & 0.38         & 0.46         \\ \cline{2-7} 
                                     & KGBugLocator   & 0.43           & 0.69           & 0.75            & 0.40         & 0.47         \\ \cline{2-7} 
                                     & BL-GAN         & 0.30           & 0.51           & 0.63            & 0.32         & -            \\ \hline
\multirow{5}{*}{SWT}                 & RLocator       & 0.30           & 0.51           & 0.58            & 0.42         & 0.44         \\ \cline{2-7} 
                                     & DeepLoc        & 0.39           & 0.66           & 0.77            & 0.40         & 0.49         \\ \cline{2-7} 
                                     & CAST           & 0.37           & 0.70           & 0.82            & 0.42         & 0.50         \\ \cline{2-7} 
                                     & KGBugLocator   & 0.38           & 0.71           & 0.83            & 0.43         & 0.51         \\ \cline{2-7} 
                                     & BL-GAN         & -              & -              & -               & -            & -            \\ \hline
\multirow{5}{*}{Tomcat}              & RLocator       & 0.39           & 0.55           & 0.68            & 0.47         & 0.51         \\ \cline{2-7} 
                                     & DeepLoc        & 0.54           & 0.72           & 0.81            & 0.56         & 0.62         \\ \cline{2-7} 
                                     & CAST           & 0.50           & 0.76           & 0.82            & 0.55         & 0.61         \\ \cline{2-7} 
                                     & KGBugLocator   & 0.51           & 0.75           & 0.82            & 0.56         & 0.62         \\ \cline{2-7} 
                                     & BL-GAN         & 0.41           & 0.63           & 0.74            & 0.45         & -            \\ \hline
\end{tabular}
\label{table:result2}
\end{table*}

==> Tables/result_table_inside.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[tb!]
\centering
\caption{RLocator performance.}
\setlength\tabcolsep{1.5pt}
\begin{tabular}{l|l|r|r}

\toprule
\textbf{Project}                & \textbf{Model} & \textbf{MAP}  & \textbf{MRR}  \\ 
\midrule
\multirow{8}{*}{\rotatebox[origin=c]{90}{AspectJ}}             & RLocator       & \begin{tabular}{|c|c|c|}
\hline
\textbf{Max}            & \textbf{Mid}            & \textbf{Min}         \\ \hline
\multicolumn{1}{|r|}{0.57} & \multicolumn{1}{r|}{0.47} & \multicolumn{1}{r|}{0.47} \\ \hline
\end{tabular} & \begin{tabular}{|c|c|c|}
\hline
\textbf{Max}            & \textbf{Mid}            & \textbf{Min}         \\ \hline
\multicolumn{1}{|r|}{0.59} & \multicolumn{1}{r|}{0.5} & \multicolumn{1}{r|}{0.5} \\ \hline
\end{tabular} \\  
                                     & BugLocator     & 0.22          & 0.41          \\ 
                                     & DeepLoc        & 0.42          & 0.51          \\  
                                     & CAST           & 0.42          & 0.54          \\  
                                     & KGBugLocator   & 0.42          & 0.55          \\  
                                     & BL-GAN         & 0.34          & -             \\ 
                                     & FBL-BERT       & 0.08          & 0.17          \\ 
                                     & FLIM           & 0.39          & 0.48          \\ \midrule
\multirow{8}{*}{\rotatebox[origin=c]{90}{Birt}}                & RLocator       & \textbf{0.47} & \textbf{0.49} \\  
                                     & BugLocator     & 0.30             & 0.35            \\  
                                     & BugLocator     & 0.30             & 0.35            \\  
                                     & DeepLoc        & -             & -             \\  
                                     & CAST           & -             & -             \\  
                                     & KGBugLocator   & -             & -             \\  
                                     & BL-GAN         & -             & -             \\  
                                     & FBL-BERT       & -             & -             \\  
                                     & FLIM           & 0.21          & 0.27          \\ \midrule
\multirow{8}{*}{\rotatebox[origin=c]{90}{\shortstack{Eclipse\\Platform UI}}} & RLocator       & \textbf{0.55} & \textbf{0.59} \\  
                                     & BugLocator     & 0.30          & 0.41          \\  
                                     & DeepLoc        & 0.43          & 0.53          \\  
                                     & CAST           & -             & -             \\  
                                     & KGBugLocator   & -             & -             \\  
                                     & BL-GAN         & 0.32          & -             \\  
                                     & FBL-BERT       & -             & -             \\  
                                     & FLIM           & 0.48          & 0.55          \\ \midrule
\multirow{8}{*}{\rotatebox[origin=c]{90}{JDT}}                 & RLocator       & \textbf{0.51} & \textbf{0.53} \\  
                                     & BugLocator     & 0.21             & 0.28             \\  
                                     & DeepLoc        & 0.44          & \textbf{0.53} \\  
                                     & CAST           & 0.47          & 0.39          \\  
                                     & KGBugLocator   & 0.4           & 0.47          \\  
                                     & BL-GAN         & 0.32          & -             \\  
                                     & FBL-BERT       & 0.06          & 0.36          \\  
                                     & FLIM           & 0.41          & 0.50          \\ \midrule
\multirow{8}{*}{\rotatebox[origin=c]{90}{SWT}}                 & RLocator       & \textbf{0.48}          & 0.51          \\  
                                     & BugLocator     & 0.45          & \textbf{0.53} \\  
                                     & DeepLoc        & 0.40          & 0.49          \\  
                                     & CAST           & 0.42          & 0.50          \\  
                                     & KGBugLocator   & 0.43          & 0.51          \\  
                                     & BL-GAN         & -             & -             \\  
                                     & FBL-BERT       & 0.12          & 0.51          \\  
                                     & FLIM           & 0.45          & 0.52          \\ \midrule
\multirow{8}{*}{\rotatebox[origin=c]{90}{Tomcat}}              & RLocator       & \textbf{0.59} & \textbf{0.62}          \\  
                                     & BugLocator     & 0.29             & 0.35             \\  
                                     & DeepLoc        & 0.56          & \textbf{0.62} \\  
                                     & CAST           & 0.55          & 0.61          \\  
                                     & KGBugLocator   & 0.56          & \textbf{0.62} \\  
                                     & BL-GAN         & 0.45          & -             \\  
                                     & FBL-BERT       & 0.13          & 0.43          \\  
                                     & FLIM           & 0.53          & 0.60          \\ 
\bottomrule
\end{tabular}

\label{table:result}
\end{table}

==> Tables/result_table_inside_v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[tb!]
\centering
\caption{RLocator performance.}
\begin{tabular}{l|l|r|r}

\toprule
\textbf{Project}                & \textbf{Model} & \textbf{MAP}  & \textbf{MRR}  \\ 
\midrule
\multirow{8}{*}{AspectJ}             & RLocator       & [0.57, 0.47,0.47]& [0.59, 0.5,0.5] \\  
                                     & BugLocator     & 0.22          & 0.41          \\ 
                                     & DeepLoc        & 0.42          & 0.51          \\  
                                     & CAST           & 0.42          & 0.54          \\  
                                     & KGBugLocator   & 0.42          & 0.55          \\  
                                     & BL-GAN         & 0.34          & -             \\ 
                                     & FBL-BERT       & 0.08          & 0.17          \\ 
                                     & FLIM           & 0.39          & 0.48          \\ \midrule
\multirow{8}{*}{Birt}                & RLocator       & \textbf{0.47} & \textbf{0.49} \\  
                                     & BugLocator     & 0.30             & 0.35            \\  
                                     & BugLocator     & 0.30             & 0.35            \\  
                                     & DeepLoc        & -             & -             \\  
                                     & CAST           & -             & -             \\  
                                     & KGBugLocator   & -             & -             \\  
                                     & BL-GAN         & -             & -             \\  
                                     & FBL-BERT       & -             & -             \\  
                                     & FLIM           & 0.21          & 0.27          \\ \midrule
\multirow{8}{*}{\shortstack{Eclipse\\Platform UI}} & RLocator       & \textbf{0.55} & \textbf{0.59} \\  
                                     & BugLocator     & 0.30          & 0.41          \\  
                                     & DeepLoc        & 0.43          & 0.53          \\  
                                     & CAST           & -             & -             \\  
                                     & KGBugLocator   & -             & -             \\  
                                     & BL-GAN         & 0.32          & -             \\  
                                     & FBL-BERT       & -             & -             \\  
                                     & FLIM           & 0.48          & 0.55          \\ \midrule
\multirow{8}{*}{JDT}                 & RLocator       & \textbf{0.51} & \textbf{0.53} \\  
                                     & BugLocator     & 0.21             & 0.28             \\  
                                     & DeepLoc        & 0.44          & \textbf{0.53} \\  
                                     & CAST           & 0.47          & 0.39          \\  
                                     & KGBugLocator   & 0.4           & 0.47          \\  
                                     & BL-GAN         & 0.32          & -             \\  
                                     & FBL-BERT       & 0.06          & 0.36          \\  
                                     & FLIM           & 0.41          & 0.50          \\ \midrule
\multirow{8}{*}{SWT}                 & RLocator       & \textbf{0.48}          & 0.51          \\  
                                     & BugLocator     & 0.45          & \textbf{0.53} \\  
                                     & DeepLoc        & 0.40          & 0.49          \\  
                                     & CAST           & 0.42          & 0.50          \\  
                                     & KGBugLocator   & 0.43          & 0.51          \\  
                                     & BL-GAN         & -             & -             \\  
                                     & FBL-BERT       & 0.12          & 0.51          \\  
                                     & FLIM           & 0.45          & 0.52          \\ \midrule
\multirow{8}{*}{Tomcat}              & RLocator       & \textbf{0.59} & \textbf{0.62}          \\  
                                     & BugLocator     & 0.29             & 0.35             \\  
                                     & DeepLoc        & 0.56          & \textbf{0.62} \\  
                                     & CAST           & 0.55          & 0.61          \\  
                                     & KGBugLocator   & 0.56          & \textbf{0.62} \\  
                                     & BL-GAN         & 0.45          & -             \\  
                                     & FBL-BERT       & 0.13          & 0.43          \\  
                                     & FLIM           & 0.53          & 0.60          \\ 
\bottomrule
\end{tabular}

\label{table:result}
\end{table}

==> code_example.tex <==
\begin{lstlisting}[caption={Example code creating nested exception},captionpos=b, language=Java, label={lst:code},breaklines=True]
public class NestedException{

   public static void main(String[] args) {
       String [] input = {"adwd", "d3d3", null};
       for (String item: input) {
           System.out.println(getLength(item));
       }
    }
    public static int getLength(String text) {
           return strip(text).length();
    }

    public static String strip(String text) {
        return text.strip();
    }
}

Exception in thread "main" java.lang.NullPointerException: Cannot invoke "String.strip()" because "<parameter1>" is null
at NestedException.strip(NestedException.java:15)
at NestedException.getLength(NestedException.java:11)
at NestedException.main(NestedException.java:7)
\end{lstlisting}
